Hyperbolic Distance versus Quasihyperbolic Distance in Plane Domains

We examine Euclidean plane domains with their hyperbolic or quasihyperbolic distance. We prove that the associated metric spaces are quasisymmetrically equivalent if and only if they are bi-Lipschitz equivalent. On the other hand, for Gromov hyperbolic domains, the two corresponding Gromov boundaries are always quasisymmetrically equivalent. Surprisingly, for any finitely connected hyperbolic domain, these two metric spaces are always quasiisometrically equivalent. We construct an example where the spaces are not quasiisometrically equivalent.

==> planar-prelims.tex <==
% prelims.tex -- created 3 March 2016
%%=========================================%%
%% prelims section for hk-geodesics paper  %%  GOTTA EDIT FOR CURRENT PAPER!
%%=========================================%%
%
% edit history
%    --
%%=========================================%%
\section{Preliminaries}  \label{S:Prelims} %%
%%=========================================%%
%
%----------------------------------------------------%
%\subsection{General Information}  \label{s:general} %
%----------------------------------------------------%
We work in the Euclidean plane, and on the Riemann sphere, which we identify, respectively, with the complex number field $\mfC$ and its one-point extension $\RS:=\mfC\cup\{\infty\}$.  Everywhere $\Om$ is a domain (i.e., an open connected set) and $\Om^c:=\mfC\sm\Om$ and $\bOm$ denote the complement and boundary (respectively) of $\Om$ \wrt the plane.  


We also always assume that $\Om^c\cup\{\infty\}$ contains at least three points; such an $\Om$ is usually dubbed a \emph{hyperbolic domain}.

%%%We write $C=C(D,\dots)$ to indicate a constant $C$ that depends only on the data $D,\dots$.  In some cases we write $K_1\lex K_2$ to indicate that $K_1\le C\,K_2$ for some computable constant $C$ that depends only on the relevant data, and $K_1\eqx K_2$ means $K_1\lex K_2\lex K_1$.

The Euclidean line segment joining two points $a,b$ is $[a,b]$, and $(a,b)=[a,b]\sm\{a,b\}$.  The open and closed Euclidean disks, and the circle, centered at the point $a\in\mfC$ and of radius $r>0$, are denoted by $\D(a;r)$ and $\D[a;r]$ and $\mfS^1(a;r)$ respectively, and $\mfD:=\D(0;1)$ is the unit disk.  We also define
\[
  \Co:=\mfC\sm\{0\} \,,\quad \Cab:=\mfC\sm\{a,b\} \,,\quad \Do:=\mfD\sm\{0\} \,, \quad \Do(a;r):=\D(a;r)\sm\{a\}\,;
\]
the definition of $\Cab$ is for distinct points $a$, $b$ in $\mfC$.

The quantity $\del(z)=\del_\Om(z):=\dist(z,\bOm)$ is the Euclidean distance from $z\in\mfC$ to the boundary of $\Om$, and $1/\del$ is the scaling factor (aka, metric-density) for the so-called \emph{quasihyperbolic} metric $\del^{-1}ds$ on $\Om\subset\mfC$; see \rf{ss:k defn}.  We make frequent use of the notation
\begin{gather*}
  \D(z)=\D_{\Om}(z):=\D(z;\del(z))=\D(z;\del_\Om(z))
  \intertext{for the maximal Euclidean disk in $\Om$ centered at a point $z\in\Om$, and then}
  \B(z)=\B_\Om(z):=\bd\D(z)\cap\bOm = \mfS^1(z;\del(z))\cap\bOm
\end{gather*}
is the set of all nearest boundary points for $z$.

We denote the usual \emph{chordal} and \emph{spherical} distances on $\RS$ by $\chi$ and $\sig$, respectively.  Thus $\sig$ is the length distance associated with $\chi$, and $\chi\le\sig\le(\pi/2)\chi$; in fact, $\chi=2\sin(\sig/2)$.\footnote{This of course follows at once when we identify $\RS$ with the unit sphere in $\mfR^3$ where we find that $\sig(u,v)$ is just the angle between $u,v$.}

Each of the metric spaces $(\Om,\ed),(\Om,\chi),(\Om,\sig)$ has an associated length distance, although the latter two are equal.  We write $l=l_\Om$ for the intrinsic (aka, inner) Euclidean length distance and $\lh=\lh_\Om$ for the intrinsic chordal/spherical length distance, and then $\Om_l:=(\Om,l)$ and $\Om_{\lh}:=(\Om,\lh)$ are the corresponding length spaces.  See for example \cite{DAH-diam-dist}.

It is also convenient to let $\chi(z)$ and $\sig(z)$ denote the chordal and spherical distances from $z$ to $\hat{\bd}\Om$.

%----------------------------------------------------------%
\subsection{Conformal Metrics}      \label{s:cfml metrics} %
%----------------------------------------------------------%
\flag{Below from hk-geos}
We call $\rho\,ds=\rho(z)|dz|$ a \emph{conformal metric} on $\Om$ provided $\rho$ is a positive continuous function defined on $\Om$.  Below we consider the hyperbolic and quasihyperbolic metrics.  Each conformal metric $\rho\,ds$ induces a length distance $d_\rho$ on $\Om$ that is defined by
\[
  d_\rho(a,b):=\inf_\gam \ell_\rho(\gam) \quad\text{where}\quad \ell_\rho(\gam):= \int_\gam \rho\, ds
\]
and where the infimum is taken over all rectifiable paths $\gam$ in $\Om$ that join the points $a,b$.  We call $\gam$ a \emph{$\rho$-geodesic} if $d_\rho(a,b)=\ell_\rho(\gam)$\footnote{Note that this agrees with the definition given in \rf{s:P&Gs}.}; these need not be unique.  We often write $[a,b]_\rho$ to indicate a $\rho$-geodesic with endpoints $a,b$, but one must be careful with this notation since these geodesics need not be unique.  When $z$ is a fixed point on a given geodesic $[a,b]_\rho$, we write $[a,z]_\rho$ to mean the subarc of the given geodesic from $a$ to $z$.

We note that the ratio $\rho\,ds/\sig\,ds$ of two conformal metrics is a well-defined positive function on $\Om$.  We write $\rho\le C\,\sig$ to indicate that this metric ratio is bounded above by $C$.

%------------------------------------------------------------------------%
\subsubsection{Hyperbolic and QuasiHyperbolic Metrics}    \label{ss:h&k} %
%------------------------------------------------------------------------%
Every hyperbolic plane domain carries a unique metric $\lam\,ds=\lam_\Om ds$ which enjoys the property that its pullback

blah blah blah

Some useful lemmas.....


%::::::::::::::::::::::::::::::::::%
\begin{lma} \label{L:cfml metrics} %
%::::::::::::::::::::::::::::::::::%
Let $\rho\,ds$ and $\sig\,ds$ be conformal metrics on some plane domain $\Om$.  Then the identity map
\[
  \Om_\rho\xra{\id}\Om_\sig \quad\text{is $1$-QC}\,.
\]
Suppose $\Om_\rho\xra{f}\Om_\sig$ is $\eta$-QS. Then $f$ induces a map
\[
  \Om\xra{f}\Om \quad\text{which is $\eta(1)$-QC}\,.
\]
\end{lma} %::::::::::::::::::::::::%
%>>>>>>>>>>>>%
\begin{proof}%
%>>>>>>>>>>>>%
%<<<<<<<<<<%
\end{proof}%
%<<<<<<<<<<%
Careful: in the above, $\eta(1)$ is the metric (aka, linear) dilatation for $f$, not the geometric dilatation.  One the other hand, below $K$ is surely the geometric dilatation.

In \cite[Theorem~3]{GO-unif}, Gehring and Osgood proved the following, which says that \qc\ \homeo s are rough \qiy s.
%................................%
\begin{fact}  \label{F:GO-k-RQI} %
%................................%
For each $K\ge1$ there is a constant $C=C(K)$ such that for any $K$-QC $\Om\xra{f}\Om'$ \homeo\ between two proper plane domains,
\[
  \forall\; a,b\in\Om\,, \quad k'\bigl(f(a),f(b)\bigr) \le C \max\{k(a,b),k(a,b)^p\}
\]
where $p:=K^{-1}$.
%..........%
\end{fact} %
%..........%

%----------------------------------------------------------%
\subsection{Annuli, Cores, \& Collars}      \label{s:anns} %
%----------------------------------------------------------%
The Euclidean annulus $A:=\{z\in\mfC :  r<|z-o|<R\}$ has \emph{center} $c(A):=o\in\mfC$ and \emph{conformal modulus} $\md(A):=\log(R/r)$; if $r=0$ or $R=\infty$, we say that $A$ is a \emph{degenerate annulus} and set $\md(A):=\infty$.\footnote{We also define $\md(\cA)=\md(A)$}   We call $\mfS^1(A):=\mfS^1(o;\sqrt{rR})$ the \emph{conformal center circle} of $A$; $A$ is symmetric about this circle.  The \emph{inner} and \emph{outer boundary circles} of $A$ are, respectively,
\[
  \bdi A:=\mfS^1(o;r) \quad\text{and}\quad  \bdo A:=\mfS^1(o;R)\,.
\]
A point $z$ is \emph{inside} (resp., \emph{outside}) $A$ \ifff $z\in\B[o;r]$ (resp., $z\in\mfC\sm\B(o;R)$); that is, $z$ is inside (or outside) $A$ \ifff $z$ is inside $\bdi A$ (or outside $\bdo A$).

It is convenient to introduce the notation
%%% \begin{gather*}----this eats my footnote :-((
%%%\begin{gather*}
%%%  A=\A(o;d,m):=\{z\in\mfC : d\,e^{-m}<|z-o|<d\,e^m\}
%%%  \intertext{and}
%%%  \A[o;d,m]:=\{z\in\mfC : d\,e^{-m}\le |z-o|<d\le e^m\}\,.
%%%  \intertext{Then}
%%%  \mfS^1(A)=\mfS^1(o;d)\,,\quad \bdi A=\mfS^1(o;d\,e^{-m})\,, \quad  \bdo A=\mfS^1(o;d\,e^m)\,.
%%%\end{gather*}
\[
  A=\A(o;d,m):=\{z\in\mfC : d\,e^{-m}<|z-o|<d\,e^m\}
  \quad\text{and}\quad
  \A[o;d,m]:=\overline{\A(o;d,m)}\,. %%%\{z\in\mfC : d\,e^{-m}\le |z-o|<d\le e^m\}\,.
\]
Then $\mfS^1(A)=\mfS^1(o;d), \bdi A=\mfS^1(o;d\,e^{-m}), \bdo A=\mfS^1(o;d\,e^m)$; here $o=c(A), d>0, m>0$\footnote{However, it is useful to define $\A(o;d,0):=\mfS^1(o;d)$ and to say that this `thin annulus' has \emph{zero} modulus.}, and $\md(A)=2m$.   See \rf{f:A(o;d,m)}.

We call $A':=\{z\in\mfC :  r'<|z-o'|<R'\}$ a \emph{subannulus of $A$} provided
\[
  A'\subset A \quad\text{and}\quad  o'\in\B[0;r]\subset\B(o';r')\,.
\]
%%% when this holds, we write $A'\subann A$.
Two annuli are \emph{concentric} if they have a common center, and $A'$ is a \emph{concentric subannulus of $A$}, denoted by $A'\csubann A$, provided $A'$ and $A$ are concentric and $A'$ is a subannulus of $A$.

An annulus $A$ \emph{separates} $E$ if each of the components of $A^c$ contains points of $E$; thus when $A$ separates $\{a,b\}$, one of $a$ or $b$ lies inside $A$ and the other lies outside $A$, and if $A$ does not meet nor separate $\{a,b\}$, then $a$ and $b$ are \emph{on the same side} of $A$.  Evidently, if $A'$ is a subannulus of $A$, then $A'$ separates the boundary circles of $A$.

We define
\begin{align*}
  \mcA(m)      &:=\{A  \mid  \text{$A$ is an Euclidean annulus with $\md(A)>m$}\}\,, \\
  \mcA_\Om     &:=\{A  \mid  \text{$A$ is an Euclidean annulus in $\Om$ with $c(A)\in\Om^c$}\}\,, \\
%%%  \mcA(a,b)    &:=\{A  :  \text{$A$ is an Euclidean annulus that separates $\{a,b\}$}\}\,,
%%%  \intertext{and then}
  \mcA^1_\Om   &:=\{A\in\mcA_\Om  \mid  \bA\cap\bOm\ne\emptyset\}\,,  \\
  \mcA^2_\Om   &:=\{A\in\mcA_\Om  \mid  \bdi A\cap\bOm\ne\emptyset\ne\bdo A\cap\bOm\}\,,  \\
  \mcA_\Om^{s}(m)     &:=\mcA^s_\Om\cap\mcA(m) \quad\text{for $s\in\{\;\;,1,2\}$}\,.
%%%  \intertext{and}
%%%  \mcA_\Om(m)     &:=\mcA_\Om\cap\mcA(m) \quad\text{and}\quad \mcA_\Om(a,b)=\mcA_\Om\cap\mcA(a,b)\,\\
%%%  \mcA^2_\Om(a,b) &:=\mcA^2_\Om\cap\mcA(a,b) \quad\text{and}\quad \mcA^2_\Om(a,b;m):=\mcA^2_\Om(a,b)\cap\mcA(m)\,.
\end{align*}
The requirement $c(A)\in\Om^c$ means, essentially, that $A$ separates $\Om^c\cup\{\infty\}$.
%%%, but here we are taking complements (for both $A^c$ and $\Om^c$) \wrt the extended plane.

%%%  Also, we say that $\gam$ \emph{bounces off $A$} if
%%%\[
%%%  |\gam|\cap A \ne\emptyset = |\gam|\cap\mfS^1(A)= \bd\gam\cap A \,.
%%%\]
%%%\flag{We could introduce a parameter $q$ and ask that $|\gam|$ not meet the middle $q$-core of $A$.  I originally used this terminology as part of the ABC property, but now?  I guess that we do not use this anywhere.}

%***************%
% Figure 1(a,b) % Center \& boundary circles of A(0;d,m); core_q(A) and its collars relative to A
%***************%
\begin{figure}
\begin{subfigure}[b]{0.48\textwidth}
\begin{tikzpicture}[scale=1.2,every text node part/.style={align=center}]
%  \draw[help lines, dashed] (-3.9,-3.9) grid (3.9,3.9);

% draw and label boundary circles for annulus A
  \node at (0,0) {\scriptsize$o$};
  \foreach \r in {1/3,3}{\draw  circle (\r);}
  \node[below] at (0,3) {\footnotesize$\bdo A$};
  \node at (20:0.7) {\footnotesize$\bdi A$};

% use even-odd-rule to shade A(How does this work??)
  \path [draw=none,fill=gray, fill opacity = 0.1,even odd rule]  circle (3) circle (1/3);

% label A and its modulus of A
  \node[draw,rounded corners,inner sep=3pt,fill=white] at (0,1.8) {$A=\A(o;d,m)$};
  \draw[<->,thin] (-45:1/3) -- (-45:3);
  \node[draw,circle,fill=white,inner sep=1pt] at (-45:5/3) {\small$2m$};

% draw and label center circle, radii
  \draw[dashed,thick] circle (1);
  \node[below,rounded corners,inner sep=1pt,fill=white] at (120:1.2) {\footnotesize$\mfS^1(A)$};
  \draw[->] (0,0) -- (-90:3);  \node [right] at (-90:2) {$\scriptstyle de^{m}$};
  \draw[->] (0,0) -- (-135:1);  \node at (-135:1.2) {\scriptsize$d$};
  \draw[->] (0,0) -- (-1/3,0);  \node at (-0.35,0.15) {\scriptsize$de^{-m}$};

% indicate the modulus of A
  \node[draw,rounded corners,inner sep=1pt,fill=white] at (-135:1.9) {\footnotesize$\md(A)=2m$};
\end{tikzpicture}
\caption{center \& boundary circles of $\A(0;d,m)$}\label{f:A(o;d,m)}
\end{subfigure}
%*****************************************************************************%
\begin{subfigure}[b]{0.48\textwidth}
\begin{tikzpicture}[scale=1.2,every text node part/.style={align=center}]
%  \draw[help lines, dashed] (-3.9,-3.9) grid (3.9,3.9);
% draw center and boundary circles for annulus A and its core
  \node at (0,0) {\scriptsize$o$};
  \foreach \r in {1/3,2/3,3/2,3}{%
    \draw  circle (\r);
  }

% using even-odd-rule to shade annuli (How does this work??)
  \path [draw=none,fill=gray, fill opacity = 0.1,even odd rule]  circle (3) circle (1/3);
  \path [draw=none,fill=blue, fill opacity = 0.15,even odd rule]  circle (3/2) circle (2/3);

% label A, its core, and the modulus of A and collar
  \node [draw,rounded corners,inner sep=3pt,fill=white] at (135:2.25) {$A$};
  \node [draw,rounded corners,inner sep=3pt,fill=white,text=blue] at (55:2.12) (QC) {\footnotesize $\core_q(A)$};
  \draw [->,thick] (QC) -- (45:1);

  \draw[<->,thin] (-1/3,0) -- (-3,0);
  \node[draw,circle,fill=white,inner sep=1pt] at (-5/3,0) {\small$2m$};

  \draw[<->,thin] (3/2,0) -- (3,0);
  \node[draw,circle,fill=white,inner sep=1pt] at (9/4,0) {\small$q$};

  \node[draw,rounded corners,fill=white,inner sep=2pt] at (0,-1.95) (BC) {\scriptsize collars of {\dkblue$\core_q(A)$} rel $A$\\[-2mm] \scriptsize both have modulus $q$};
  \draw[->,thick] (BC) -- (0.5,0);  \draw[->,thick] (BC) -- (-30:2.25);
\end{tikzpicture}
\caption{$\core_q(A)$ and its collars relative to $A$}\label{f:q-core(A)}
\end{subfigure}
\caption{The annulus $\A(o;d,m)$ and its $q$-core; here \protect\raisebox{-2mm}{\protect\tikz\protect\node[draw,circle,inner sep=1pt]{\small$2m$};} indicates the modulus}\label{f:annuli}
%************%
\end{figure} %
%************%

%---------------------------------------------------------%
\subsubsection{Annulus Cores \& Collars}  \label{ss:cores}%
%---------------------------------------------------------%
For a non-degenerate annulus $A$ and $m\in(0,\half\md(A))$, there is a unique concentric subannulus of $A$ that has modulus $2m$ and center circle $\mfS^1(A)$.  Such a subannulus is an example of a \emph{middle core} of $A$, and the complement (in $A$) of its closure is the union of two concentric subannuli of $A$, each of modulus $\half\md(A)-m$, that we call its (\emph{inner} and \emph{outer}) \emph{collars} relative to $A$.

Controlling the size of these collars is crucial for our purposes.  Given $q\in(0,\half\md(A))$, we define $\core_q(A)$---which we call the \emph{core of $A$ with collar parameter $q$}---to be the concentric subannulus of $A$ with the same center circle as $A$ and such that $\md(\core_q(A))=\md(A)-2q$.  Thus $A\sm\overline\core_q(A)$ is the union of two concentric subannuli of $A$ each of modulus $q$; these are the (\emph{inner} and \emph{outer}) \emph{collars of $\core_q(A)$ relative to $A$}.  See \rf{f:q-core(A)}.

We often describe $\core_q(A)$ as the \emph{middle $q$-core} of $A$, but one must remember that $q$ is the collar parameter; that is, $q$ gives the size of the collars of the core, relative to $A$.  For example, the $\log2$-core of $\{r<|z|<R\}$ is $\{2r<|z|<R/2\}$, and its $q$-core is $\{re^{q}<|z|<Re^{-q}\}$.  When $A=\A(o;d,m)$ and $0<q<m$,
\[
  \core_q(A)=\A(o;d,m-q)  \quad\text{and}\quad  \overline\core_q(A)=\A[o;d,m-q]\,.
\]

It is useful to have a similar notion for degenerate annuli.  To this end, we define
\[
  \core_q(A):=
    \begin{cases}
      \D_*(o;e^{-q}R)       &\text{when $A=\D_*(o;R)$}\,,       \\
      \mfC\sm\D[o;e^{q}R]   &\text{when $A=\mfC\sm\D[o;R]$}\,.  \\
    \end{cases}
\]
Here in both cases $\core_q(A)\csubann A$ but now $A\sm\overline\core_q(A)$ is a single annulus of modulus $q$ (and $q>0$ can be arbitrary).

We adopt the convention that whenever we write $\core_q(A)$ we have $0<q<\half\md(A)$.  With this in mind, $A\csubann B$ implies $\core_q(A)\csubann\core_q(B)$.  Also, if $q<r$, $\overline\core_r(A)\csubann\core_q(A)$, and always $\core_q\core_r(A)=\core_{q+r}(A)=\core_r\core_q(A)$.

It is convenient to have the notion of the core of a closed annulus, so we define $\core_q(\cA):=\overline\core_q(A)$.  Thus the core of an open (or closed) annulus is a concentric open (or closed) subannulus.

At times we employ a dual (or inverse) notion of a core.  The \emph{$r$-banding} of an annulus $A$ is the unique concentric superannulus $\band_r(A)\supset A$ with the property that $\core_r\band_r(A)=A$.  Again, $\band_r(A)$ is an open or closed annulus depending upon whether $A$ is open or closed.  We also define $\band_r\bigl(\mfS^1(o;d)\bigr):=\A(o;d,r)$ (here the $r$-banding of a ``closed zero modulus annulus'' is an open annulus).  Evidently, for all $r>0$,
\begin{align*}
  \band_r\A(o;d,m) &= \A(o;d,m+r)\,, \\
  \md\band_r(A) &= \md(A)+2r\,,      \\
  \core_r\band_r(A)&=A=\band_r\core_r(A)\,.
\end{align*}
In fact, $\core_q\band_r(A)=\band_r\core_q(A)=\core_t\band_s(A)$; here the final equality requires $r-q=s-t$ (amongst other conditions too), and we leave it to the reader to recognize the various restrictions on the core parameters $q,r,s,t$.

%----------------------------------------------------%
\subsubsection{Crossing an Annulus}  \label{ss:cross}%
%----------------------------------------------------%
%Let $A$ be an annulus and $\gam$ be
A path $\gam$ \emph{meets} or \emph{misses} an annulus $A$ depending on whether $|\gam|\cap A\ne\emptyset$ or $|\gam|\cap A=\emptyset$, and $\gam$ \emph{crosses $A$} if
\[
  |\gam|\cap\bdi A\ne\emptyset\ne|\gam|\cap\bdo A
\]
and $\gam$ \emph{does not cross $A$} if one of the above intersections is empty.  Next, $\gam$ \emph{crosses $A$ $n$ times} if there are non-overlapping subpaths $\gam_1,\dots,\gam_n$\footnote{We can arrange that the terminal point of $\gam_{i-1}$ and initial point of $\gam_i$ lie on the same side of $A$.} of $\gam$ such that each $\gam_i$ crosses $A$, and \emph{$\gam$ crosses $A$ exactly $n$ times} if it crosses $n$ times but not $n+1$ times.  Evidently, if $A$ separates the endpoints of $\gam$, then $\gam$ crosses $A$.

%---------------------------------------------------------%
\subsection{$\chi$-Arc Crosscuts}      \label{s:chi arcs} %
%---------------------------------------------------------%
We employ the following construction in numerous circumstances.  Given two points $a,b$ on some circle $C$, we write $\kap_{ab}$ for the \emph{shorter circular arc in $C$ from $a$ to $b$}; when $a,b$ are diametrically opposite, $\kap_{ab}$ can be either semi-circle.  Next, suppose $a,b$ are points that each lie on one of the boundary circles of an annulus $A$; say $a$ lies in $C_a$ and $b$ lies in $C_b$ where $\bA=C_a\cup C_b$.  Let $c$ and $d$ be the radial projections (\wrt the center of $A$) of $b$ onto $C_a$ and $a$ onto $C_b$,  respectively.  Then
\begin{subequations}\label{E:chi}
\begin{gather}
   \chi_{ab}:=\kap_{ac}\star[c,b] \quad\text{is the \emph{circular-arc-segment} from $a$ through $c$ to $b$.}  \label{E:chi-ab}
   \intertext{and}
   \chi_{ba}:=\kap_{bd}\star[d,a] \quad\text{is the \emph{circular-arc-segment} from $b$ through $d$ to $a$.}  \label{E:chi-ba}
\end{gather}
\end{subequations}
Note that we also have the reverse paths, $\chi^{-1}_{ab}=[b,c]\star\kap_{ca}$ and $\chi^{-1}_{ba}=[a,d]\star\kap_{db}$ which are \emph{segment-circular-arcs} from $b$ through $c$ to $a$ and from $a$ through $d$ to $b$ respectively.  See the proofs of \rfs{TT:unif} and \ref{TT:inner} where we make extensive use of such $\chi$-arcs.

All of these $\chi$-arcs are crosscuts of certain annuli, and it is easy to check that $\chi$-arcs are quasiconvex.  In fact, a $\chi$-arc that joins the boundary circles of a fat annulus in $\mcA_\Om$ is a uniform arc in $\Om$; indeed, these are even cone arcs.

%::::::::::::::::::::::::::::::::%
\begin{lma}  \label{L:chi props} %
%::::::::::::::::::::::::::::::::%
Let $a,b\in\Co$ with $0<|a|\le|b|$.  Let $\chi:=\chi_{ab}$ be the circular-arc-segment path from $a$ through $c:=\bigl(|a|/|b|\bigr)b$ to $b$ as described above.  Then
\addtocounter{equation}{-1}  % want subeqn labels below to match Lemma label
\begin{subequations}\label{E:chi ests}
  \begin{alignat}{2}
    &\forall\, x,y\in|\chi|\,, &\quad&\ell(\chi[x,y])\le3|x-y|\,.      \label{E:chi qcx}
    \intertext{If $a,b\in\core_{\log2}(A)$ for some $A=\A(0;d,m)\in\mcA_\Om(\log4)$, then also}
    &\forall\, z\in|\chi|\,,   &&\ell(\chi[z,a])\le2\pi\del(z)\,.      \label{E:chi cone}
%%% apparently \eqref{E:chi cone2} is never used!?
%%%    \intertext{and}
%%%    &\forall\, z\in|\chi|\,,   &&\ell(\chi[z,b])\le2(C+\pi-1)\del(z) \;\text{provided $|z|\ge|b|/C$}.  \label{E:chi cone2}
  \end{alignat}
\end{subequations}
\end{lma} %::::::::::::::::::::::%
%>>>>>>>>>>>>%
\begin{proof}%
%>>>>>>>>>>>>%
We have $\chi:=\chi_{ab}=\kap\star[c,b]$, where $\kap=\kap_{ac}$.  Put $\tha:=|\Arg(b/a)|=|\Arg(c/a)|$.  According to the Law of Cosines,
\begin{gather*}
  |a-c|^2=2|a|^2(1-\cos\tha)\,, \quad\text{so}\quad \cos\tha=1-\frac{|a-c|^2}{2|a|^2}
  \intertext{and therefore}
 \begin{align*}
  |a-b|^2&=|a|^2+|b|^2-2|a||b|\cos\tha=|a|^2+|b|^2-2|a||b|\biggl(1-\frac{|a-c|^2}{2|a|^2} \biggr) \\
     &= |a|^2+|b|^2-2|a||b|+|b|\frac{|a-c|^2}{2|a|} = \bigl(|a|-|b|\bigr)^2 + \frac{|b|}{|a|}\,|a-c|^2 \ge |a-c|^2\,.
 \end{align*}
  \intertext{Thus}
  \ell(\kap)\le\frac{\pi}2\,|a-c|\le\frac{\pi}2\,|a-b|
  \intertext{and hence}
  \ell(\chi)=\ell(\kap)+\bigl(|b|-|a|\bigr)\le\bigl(\frac{\pi}2\,+1\bigr)|a-b|\,. %  \qedhere
\end{gather*}
%-----following was used in geodesics paper, but not needed here
%%% If $|b|\le e|a|$, then as $\ell(\kap)\le\pi|a|$ we have $\ell(\chi)\le (\pi+e-1)|a|\le 2e|a|$.

To verify \eqref{E:chi qcx}, notice that $\chi[x,y]=\chi_{xy}$.  Assume $a,b\in\core_{\log2}(A)$ for some $A=\A(0;d,m)\in\mcA_\Om(\log4)$.  Then by \rf{L:del deep in A}, for all $z\in|\chi|$, $\del(z)\ge\half|z|$.  Thus if $z\in|\kap|$, then
\begin{gather*}
  \ell(\chi[z,a])=\ell(\kap[z,a])\le\pi|z|\le2\pi\del(z)
  \intertext{and if $z\in[c,b]$, then}
  \ell(\chi[z,a])=\ell(\kap)+\bigl(|z|-|c|\bigr)\le\pi|c|+\bigl(|z|-|c|\bigr)\le\pi|z|\le2\pi\del(z)
\end{gather*}
which establishes \eqref{E:chi cone}.
%<<<<<<<<<<%
\end{proof}%
%<<<<<<<<<<%

%::::::::::::::::::::::::::::::::%
\begin{cor}  \label{C:chi props} %
%::::::::::::::::::::::::::::::::%
For any points $z,w$ in any closed annulus that lies in $\Om$ we have
\[
  l(z,w)\le3|z-w| \quad\text{and}\quad j_\ell(z,w)\le3j(z,w)\,.
\]
\end{cor} %::::::::::::::::::::::%

%------------------------------------------------------------------------------------------------%
\subsection{Hyperbolic and QuasiHyperbolic Metrics, Distances, Geodesics}      \label{s:h-k MDG} %
%------------------------------------------------------------------------------------------------%
Every hyperbolic plane domain carries a unique metric $\lam\,ds=\lam_\Om ds$ which enjoys the property that its pullback $p^*[\lam\,ds]$, \wrt any holomorphic universal covering projection $p:\D\to\Om$, is the hyperbolic metric $\lam_\D(\zeta)|d\zeta|=2(1-|\zeta|^2)^{-1}|d\zeta|$ on $\D$.  In terms of such a covering $p$, the metric-density $\lam=\lam_\Om$ of the {\em Poincar\'e hyperbolic metric\/} $\lam_\Om ds$ can be determined from
$$
  \lam(z)=\lam_\Om(z)=\lam_\Om(p(\zeta))=2(1-|\zeta|^2)^{-1}|p'(\zeta)|^{-1}\,.
$$
Yet another description is that $\lam\,ds$ is the unique maximal (or unique complete) metric on $\Om$ that has constant Gaussian curvature $-1$.

For example, the hyperbolic metric $\lam_*ds$ on the punctured unit disk $\D_*:=\D\sm\{0\}$ can be obtained by using the universal covering $z=\exp(w)$ from the left-half-plane onto $\D_*$ and we find that
\[
  \lam_*(z)|dz|=\frac{|dz|}{|z|\bigl|\log|z|\bigr|}\,.
\]

Except for a short list of special cases, the actual calculation of any given hyperbolic metric is notoriously difficult; computing hyperbolic distances and determining hyperbolic geodesics is even harder.  Indeed, one can find a number of papers analyzing the behavior of the hyperbolic metric in a twice punctured plane.  Typically one is left with estimates obtained by using domain monotonicity and considering `nice' sub-domains and super-domains in which one can calculate, or at least estimate, the metric.

In many cases (but certainly not all), the hyperbolic metric is \BL\ equivalent to the \emph{quasihyperbolic metric} $\del^{-1}ds=|dz|/\del(z)$, where $\del=\del_\Om$, which is defined for any proper subdomain $\Om\subsetneq\mfC$.  This metric has proven useful in many areas of geometric analysis.

\medskip

The \emph{hyperbolic distance} $h=h_\Om$ and \emph{quasihyperbolic distance} $k=k_\Om$ in $\Om$ are the length distances $h_\Om:=d_{\lam}$ and $k_\Om:=d_{\del^{-1}}$ that are induced by the hyperbolic and quasihyperbolic metrics $\lam\,ds, \del^{-1}ds$ on $\Om$.  These are geodesic distances: for any points $a,b$ in $\Om$, there are always an $h$-geodesic $[a,b]_h$ and a $k$-geodesic $[a,b]_k$ joining $a,b$ in $\Om$.  These geodesics need not be unique, but they enjoy the properties that
\[
  h(a,b)=\ell_h([a,b]_h) \quad\text{and}\quad k(a,b)=\ell_k([a,b]_k)\,.
\]
Here we are writing $\ell_h$ and $\ell_k$ in lieu of $\ell_\lam$ and $\ell_{\del^{-1}}$.

We adopt the following \textbf{\emph{conventions}} throughout the remainder of this paper: the term \emph{geodesic} shall mean either a hyperbolic geodesic or a quasihyperbolic geodesic (we will explicitly say which when it is necessary to do so) and we will say that $[a,b]_g$ (for $g=h$ or $g=k$) is a geodesic to mean that it is a hyperbolic geodesic when $g=h$ and a quasihyperbolic geodesic when $g=k$.
We adopt similar conventions when discussing quasi-geodesics; see \rf{s:PAGs} for their definitions.

\medskip

An important property of hyperbolic distance is its conformal invariance.  While this does not hold for quasihyperbolic distance, it is \Mob\ quasi-invariant in the following sense; see \cite[Lemma~2.4, Corollary~2.5]{GP-qch}.  Modifications to their argument also gives quasi-invariance of the relative distances $j, j'$.

%...........................%
\begin{fact}  \label{F:kQI} %
%...........................%
Let $\RS\xra{T}\RS$ be a \MT.  Let $\Om\subsetneq\mfC$ and suppose $\Om':=T(\Om)\subset\mfC$.  Put $\del':=\del_{\Om'}, k':=k_{\Om'}$, and $j':=j_{\Om'}$.  Then
\begin{gather*}
  \forall\; z\in\Om\,, \quad  \frac1{\del(z)} \le2\,\frac{|T'(z)|}{\del'(T(z))}\,.
  \intertext{Consequently, for all rectifiable paths $\gam$ in $\Om$,}
  \half \ell_k(\gam) \le \ell_{k'}(T\comp\gam) \le 2\ell_k(\gam)\,.
  \intertext{In particular, with $a':=T(a)$ and $b':=T(b)$,}
  \forall\; a,b\in\Om\,, \quad \half k(a,b) \le k'(a',b') \le 2k(a,b)
  \intertext{and also}
  \forall\; a,b\in\Om\,, \quad \half j(a,b) \le j'(a',b') \le 2j(a,b)\,.
\end{gather*}
%..........%
\end{fact} %
%..........%

%%%%%
%%%%%%----------------------------------------------------------------%
%%%%%\subsection{The Beardon-Pommerenke Function $\bp$}  \label{s:BP} %
%%%%%%----------------------------------------------------------------%
%%%%%We desire upper and lower estimates for the hyperbolic metric.
%%%%%%%%  In general, finding lower estimates %for the hyperbolic metric seems to be the more difficult endeavor.
%%%%%These metrics are 2-bi-Lipschitz equivalent for simply connected hyperbolic plane regions; this is false for any domain with an isolated boundary point (such as the punctured unit disk).  The hyperbolic and quasihyperbolic metrics are bi-Lipschitz equivalent precisely when $\Om^c$ is uniformly perfect (cf.\ \cite{BP-beta}, \cite{Pomm-unifly-perfect1}, \cite{Pomm-unifly-perfect2}).  Beardon and Pommerenke corroborated this latter assertion as an application of their elegant result \cite[Theorem~1]{BP-beta} which says:
%%%%%\begin{noname}
%%%%%For any hyperbolic region $\Om$ in $\mfC$ and for all $z\in\Om$,
%%%%%\[
%%%%%  \frac{1}{\del(z)\bigl(\KK+\bp(z)\bigr)} \le \lam(z)  %%% \frac{\pi}{2}\;\frac{1}{\del(z) \, \bp(z)} \,.  \tag{\BPt}
%%%%%  \le \frac{\pi/2}{\del(z) \, \bp(z)} \,.  \tag{\BPt}
%%%%%\]
%%%%%\end{noname}
%%%%%\noindent
%%%%%Beardon and Pommerenke introduced the domain function $\Om\xra{\bp}\mfR$ which is defined via
%%%%%\[
%%%%%%%\begin{equation}								\label{E:beta}
%%%%%  \bp(z)=\bp_{\Om}(z):=
%%%%%  \inf_{\substack{
%%%%%    {\zeta\in\B(z)}\\
%%%%%     \xi\in\Om^c\sm\{\zeta\}}}
%%%%%    \biggl|\log\Bigl|\frac{\zeta-z}{\zeta-\xi}\Bigr|\biggr|\,;
%%%%%%%\end{equation}
%%%%%\]
%%%%%note that the infimum is restricted to nearest boundary points $\zeta\in\B(z)=\bOm\cap\bD(z)$ for $z$ (that is, $\zeta\in\bOm$ with $\del(z)=|z-\zeta|$).  Also, here
%%%%%\[\KK:= \bigl(\lam_{01}(-1)\bigr)^{-1} = \Gam^4(1/4)/\bigl(4\pi^2\bigr)=4.3768796\dots\,.\]
%%%%%
%%%%%The definition of $\bp$ is motivated by examining the standard lower bound for the hyperbolic metric on a twice punctured plane. The (\BPt) inequalities follow via domain monotonicity: the upper bound for $\lam(z)$ holds because $z$ lies on the conformal center of a certain annulus in $\Om$, and the lower bound holds because $\Om$ lies in a certain twice punctured plane.
%%%%%
%%%%%A geometric interpretation for $\bp(z)$ is seen by defining $\bp(z,\zeta)$---for points $z\in\Om$ and $\zeta\in\B(z)$---as follows:
%%%%%%%%\begin{gather*}
%%%%%\[
%%%%%  \bp(z,\zeta):=\inf_{\xi\in\Om^c\sm\{\zeta\}} \biggl|\log\Bigl|\frac{\zeta-z}{\zeta-\xi}\Bigr|\biggr|\,.
%%%%%  \qquad\text{(Thus, $\ds\bp(z)=\inf_{\zeta\in\B(z)}\bp(z,\zeta)$)}\,.
%%%%%\]%%%\end{gather*}
%%%%%We find that $2\bp(z,\zeta)$ is the conformal modulus of the maximal Euclidean annulus that is contained in $\Om$ and symmetric \wrt the circle $\mfS^1(\zeta;\del(z))$.  It follows that $2\bp(z)$ is the minimum of these numbers; so, $2\bp(z)$ is the smallest of these maximal moduli.
%%%%%
%%%%%%************%
%%%%%% BP annulus %
%%%%%%************%
%%%%%Thus we see that whenever $\bp(z)>0$, there is an annulus
%%%%%\begin{gather*}
%%%%%  \BP(z):=\A(\zeta;\del(z),\bp(z)) \in\mcA^1_\Om
%%%%%  \intertext{associated with $z$; here $\zeta\in\B(z)$ is any nearest boundary point for $z$ that realizes $\bp(z)$, and}
%%%%%  \forall\;\xi\in\bd\BP(z)\cap\bOm\,,\quad \bp(z)=\bp(z,\zeta)=\biggl|\log\Bigl|\frac{\zeta-z}{\zeta-\xi}\Bigr|\biggr|\,.
%%%%%\end{gather*}
%%%%%We call $\BP(z)$ a \emph{Beardon-Pommerenke annulus} (or briefly, a \emph{\BPt\ annulus}) associated with the point $z$; it needn't be unique.
%%%%%
%%%%%\smallskip
%%%%%
%%%%%In this paper \emph{we only care about large values} of $\bp$.  In particular, when $\bp\ge\KK$ the (\BPt) inequalities imply that
%%%%%\begin{equation}\label{E:BP est}
%%%%%  \frac1{2\,\del\,\bp} \le \lam \le \frac2{\del\,\bp}\,.
%%%%%\end{equation}
%%%%%
%%%%%In \cite[Proposition~3.3]{HB-geodesics} we established especially useful estimates for $\bp$; these say that in any annulus in $\mcA^2_\Om(8\log2)$, the domain function $\bp$ decays `linearly' as we move away from the center circle.  The assumption that both boundary circles of the annulus meet $\bOm$ is crucial for obtaining the upper bounds; when only one boundary circle has a boundary point, $\bp$ can actually increase when we move away from the center circle towards the boundary circle that does not meet $\bOm$.  Here is a summary.
%%%%%
%%%%%%............................%
%%%%%\begin{fact}  \label{F:BPEP} %
%%%%%%............................%
%%%%%Let $\A(o;d,r)\in\mcA^2_\Om(8\log2)$, so $r>\log16$. For $|t|\lex r$ and all $z\in\mfS^1(o;de^t)$, $\bp(z)\eqx r-|t|$.  More precisely, for $|t|\le r-\log16$ and $z\in\mfS^1(o;de^t)$,
%%%%%\[
%%%%%  \frac12 \lp r-|t| \rp \le \bp(z) \le2 \lp r-|t| \rp\,.
%%%%%\]
%%%%%In the above, $z\in\overline\core_{\log16}(A)$ and $t:=\log\lp|z-o|/d\rp$.  In particular:
%%%%%
%%%%%\smallskip\noindent(a)  In $\core_{\log16}(A)$, $\bp\le 2r=\md(A)$, and on $\mfS^1(A)=\mfS^1(o;d)$, $\bp\ge\half r$.
%%%%%
%%%%%\smallskip\noindent(b)  On both boundary circles $\mfS^1(o;16^{\pm1}de^{\mp r})$, $2\log2 \le \bp \le 8\log2$.
%%%%%
%%%%%\smallskip\noindent(c)  For $\log16<q<r$ we have the strict inequalities
%%%%%\[
%%%%%  \text{$\bp>\half\,q$ in $\core_q(A)$ \hspace{1em} and \hspace{1em} $\bp<2\,q$ in $\core_{\log16}(A)\sm\overline\core_q(A)$}\,.
%%%%%\]
%%%%%
%%%%%\smallskip\noindent(d)  We also have estimates for $\bp$ in annuli $A=\A(o;d,r)\in\mcA^1_\Om$, as long as we move towards the boundary circle that has a boundary point.
%%%%%%%%  To be precise, suppose $|z-o|=de^t$ with $|t|\le r-\log16$.  Then
%%%%%%%%\begin{align*}
%%%%%%%%   \bp(z) &\le2 \lp r-|t| \rp        &\text{when $t\ge0$ and $\bdo A\cap\bOm\ne\emptyset$}\,, \\
%%%%%%%%   \bp(z)& \le \lp r-|t| \rp + \log2 &\text{when $t\le0$ and $\bdi A\cap\bOm\ne\emptyset$}\,.
%%%%%%%%\end{align*}
%%%%%%..........%
%%%%%\end{fact} %
%%%%%%..........%
%%%%%
%%%%%\flag{I think we only need $-r+\log16\le t \le r-\log3$ :-)}
%%%%%
%%%%%
%%%%%Recall from above that for each $z\in\Om$ with $\bp(z)>0$ there is an associated \emph{Beardon-Pommerenke annulus}
%%%%%\[
%%%%%  \BP(z):=\A(\zeta;\del(z),\bp(z))\in\mcA^1_\Om \quad\text{(so, $\BP(z)\subset\Om$ and $\bd\BP(z)\cap\bOm\ne\emptyset$)}.
%%%%%\]
%%%%%%************************************%
%%%%%% BP annulus and enlarged BP annulus %
%%%%%%************************************%
%%%%%For our purposes, there is a second more important annulus $\A(z)$ which has the crucial property that \emph{both} of its boundary circles meet $\bOm$; this permits the use of \rf{F:BPEP}. %%% to estimate $\bp$ in $\A(z)$.
%%%%%If $\BP(z)\in\mcA^2_\Om$, %%% (i.e., if $\BP(z)$ already has the property that both of its boundary circles meet $\bOm$),
%%%%%we set $\A(z):=\BP(z)$.  Otherwise, we obtain $\A(z)$ by enlarging $\BP(z)$ until we hit $\bOm$; that is, we start with the boundary circle of $\BP(z)$ that does not meet $\bOm$ and then grow or shrink this circle (keeping its center fixed) until we hit $\bOm$.
%%%%%%%%
%%%%%%%%To be precise \flag{pictures here!?}, suppose
%%%%%%%%\begin{gather*}
%%%%%%%%  m:=\bp(a)=\biggl|\log\Bigl|\frac{\zeta-a}{\zeta-\xi}\Bigr|\biggr|
%%%%%%%%  \intertext{with $\zeta\in\B(a)$ and $\xi\in\bOm$, so}
%%%%%%%%  \BP(a)=\A(\zeta;\del(a),m)=\{z\in\mfC  :  \del(a)e^{-m}<|z-\zeta|<\del(a)e^m\}\,.
%%%%%%%%\end{gather*}
%%%%%%%%We assume one of the boundary circles of $\BP(a)$ does \emph{not} meet $\bOm$; so, $\BP(a)\in\mcA^1_\Om\sm\mcA^2_\Om$.  There are two cases depending on whether $|\zeta-\xi|=\del(a)e^m$ or $|\zeta-\xi|=\del(a)e^{-m}$.
%%%%%%%%
%%%%%%%%Assume $\xi\in\bdi\BP(a)$, so $|\zeta-\xi|=\del(a)e^{-m}$.  Put
%%%%%%%%\begin{gather*}
%%%%%%%%  R:=\sup\{r\ge\del(a)e^m : \{z\in\mfC  :  \del(a)e^{-m}<|z-\zeta|<r\}\subset\Om \}
%%%%%%%%  \intertext{and define}
%%%%%%%%  \A(a):=\{z\in\mfC  :  |\zeta-\xi| < |z-\zeta| < R\}\,.
%%%%%%%%\end{gather*}
%%%%%%%%Note that if $R=+\infty$, then $\A(a)=\mfC\sm\D[\zeta;|\zeta-\xi|]$ which should be viewed as a punctured disk on the Riemann sphere $\RS$.  Suppose $R<\infty$.  Then there exists a point $\eta\in\mfS^1(\zeta;R)\cap\bOm$, and now
%%%%%%%%\begin{gather*}
%%%%%%%%  \A(a)=\A(\zeta;d,\ups)=\{z\in\mfC  :  d e^{-\ups}<|z-\zeta|<d e^\ups\}\,,
%%%%%%%%  \intertext{where}
%%%%%%%%  d:=\lp |\zeta-\xi||\zeta-\eta| \rp^\half = \lp \del(a)e^{-m} R \rp^\half > \del(a)
%%%%%%%%  \intertext{and}
%%%%%%%%  \ups:=\log\frac{R}{d}=m+\log\frac{d}{\del(a)}>m=\bp(a)\,.
%%%%%%%%\end{gather*}
%%%%%%%%
%%%%%%%%Assume $\xi\in\bdo\BP(a)$, so $|\zeta-\xi|=\del(a)e^{m}$.  Put
%%%%%%%%\begin{gather*}
%%%%%%%%  \veps:=\inf\{0<r\le\del(a)e^{-m} : \{z\in\mfC  :  r<|z-\zeta|<\del(a)e^{m}\}\subset\Om \}
%%%%%%%%  \intertext{and define}
%%%%%%%%  \A(a):=\{z\in\mfC  :  \veps < |z-\zeta| < |\zeta-\xi|\}\,.
%%%%%%%%\end{gather*}
%%%%%%%%Now if $\veps=0$, then $\A(a)=\D_*(\zeta;|\zeta-\xi|)$ which is a punctured disk.  Suppose $\veps>0$.  Then there exists a point $\eta\in\mfS^1(\zeta;\veps)\cap\bOm$, and
%%%%%%%%\begin{gather*}
%%%%%%%%  \A(a)=\A(\zeta;d,\ups)=\{z\in\mfC  :  d e^{-\ups}<|z-\zeta|<d e^\ups\}\,,
%%%%%%%%  \intertext{where}
%%%%%%%%  d:=\lp |\zeta-\xi||\zeta-\eta| \rp^\half = \lp \del(a)e^{m} \veps \rp^\half < \del(a)
%%%%%%%%  \intertext{and}
%%%%%%%%  \ups:=\log\frac{d}{\veps}=m+\log\frac{\del(a)}{d}>m=\bp(a)\,.
%%%%%%%%\end{gather*}
%%%%%%%%
%%%%%%%%We summarize the above.
%%%%%We find that:
%%%%%\begin{itemize}
%%%%%  \item  $\A(z)\in\mcA^2_\Om$ is either a punctured disk in $\RS$ or $\A(z)=\A(\zeta;d,\ups)$ where $\zeta\in\B(z)$, $d>0$, and $\ups\ge\bp(z)$.%%%  Thus we can always talk about $\core_q\A(z)$ where either $q>0$ in the first (two) case(s) or $0<q<\ups$ in the last case.
%%%%%  \item  The point $z$ lies on the boundary of a concentric subannulus of $\A(z)$ (in fact, $z$ lies on the boundary of a collar) that has modulus $\bp(z)$.  In particular,
%%%%%  \begin{equation}\label{E:z in core bdy}
%%%%%    z\in\bd\core_{\bp(z)}\A(z)\subset\overline\core_{\bp(z)}\A(z)\,.
%%%%%  \end{equation}
%%%%%\end{itemize}
%%%%%Notice that we can only apply the \BPEP\ to obtain estimates when $\A(z)$ is non-degenerate, but when $\A(z)$ is degenerate, we actually have a precise formula for $\bp$.  For example, if say $\A(a)=\D_*(0;R)$, then for $z\in\core_{\log2}\A(a)=\D_*(0;R/2)$ we have $\bp(z)=\log(R/|z|)$.
%%%%%
%%%%%\smallskip
%%%%%
%%%%%We conclude this subsection with the following elementary, but surprisingly useful, observation; see \cite[Lemma~3.6]{HB-geodesics}.  We often apply this result to curves.
%%%%%
%%%%%%.................................%
%%%%%\begin{fact}  \label{F:bp ge tau} %
%%%%%%.................................%
%%%%%Fix $\tau>8\log2$.  Let $E$ be a connected subset of $\Om$.  Suppose that $\bp\ge\tau$ in $E$.  Then
%%%%%\[
%%%%%  E \subset \bigcap_{z\in E} \overline\core_{\tau/2}\A(z)\,.
%%%%%\]
%%%%%\end{fact} %......................%
%%%%%
%%%%%%---------------------------------------------------%
%%%%%\subsection{The Arcs Bounce or Cross Property}  \label{s:ABC} %
%%%%%%---------------------------------------------------%
%%%%%% its defn and props
%%%%%% k & h have
%%%%%A path $\mfR\supset I\xra{\gam}\Om$ has the \emph{ABC property}\footnote{\emph{ABC} is short for \emph{arcs bounce or cross}.}, with parameters $\mu>0$ and $\nu>0$, \ifff for each compact subpath $\alf$ of $\gam$ and for each annulus $A:=\A(o;d,\nu)\in\mcA_\Om$ such that $\mfS^1(A)\supset\bd\alf$, we have $|\alf|\subset\A(o;d,\mu)$; equivalently, for each circle $C$ with $\band_\nu(C)\in\mcA_\Om$, $\bd\alf\subset C\implies|\alf|\subset\band_\mu(C)$.
%%%%%
%%%%%The ABC property implies that the path can cross a moderate size annulus at most once, so if the path enters deep into an annulus, it either stays there  or it crosses (once) and never returns.  In particular, if the path goes near an ``isolated island or archipelago'' of $\Om^c\cup\{\infty\}$, then it stays near it.  Here are various precise statements of this phenomenon; see \cite[Lemma~3.7]{HB-geodesics}.
%%%%%
%%%%%%..........................%
%%%%%\begin{fact} \label{F:ABC} %
%%%%%%..........................%
%%%%%Suppose a path $\mfR\supset I\xra{\gam}\Om$ has the \emph{ABC property} with parameters $\mu\ge\nu>0$.  Let $A:=\A(o;d,m), A_\nu:=\A(o;d,\nu), A_\mu:=\A(o;d,\mu)$.  Suppose $\alf$ is a compact subpath of $\gam$.
%%%%%\begin{aenum}
%%%%%  \item  Assume $A_\nu\in\mcA_\Om$.  If $m\ge\mu$, then $\alf$ crosses $A$ at most once. %%%  If any $\rho$-geodesic crosses $A$ twice, then $m\le\mu$.  Therefore, if $m>\mu$, then every $\rho$-geodesic either crosses $A$ exactly once or does not cross $A$.
%%%%%  \item  Assume $\band_{\nu}(A)\in\mcA_\Om$.  If $\bd\alf\subset\cA$, then $|\alf|\subset\band_{\mu}(A)$.
%%%%%  \item  Assume $A\in\mcA_\Om$ and $m\ge\mu+\nu$.  Suppose $\bd\alf\cap\A_\mu=\emptyset$.  Then
%%%%%  \[
%%%%%    \text{either}\quad |\alf|\cap\mfS^1(A)=\emptyset \quad\text{or $\quad\mfS^1(A)$ separates $\bd\alf$}\,.
%%%%%  \]
%%%%%  \hspace{1.3em}In fact, if $|\alf|\cap\mfS^1(A)\ne\emptyset$, then $A_\mu$ separates $\bd\alf$.
%%%%%  \item  Assume $A\in\mcA_\Om$ and $m>2\mu$.  Suppose $\bd\alf\cap A=\emptyset$.  Then
%%%%%  \[
%%%%%    \text{either}\quad |\alf|\cap\overline\core_{2\mu}(A)=\emptyset \quad\text{or $A$ separates $\bd\alf$}\,.
%%%%%  \]
%%%%%\end{aenum}
%%%%%\end{fact} %...............%
%%%%%
%%%%%\rf{F:ABC}(d) above is the origin for the term ``ABC property''.  It says that for each sufficiently fat annulus $A\in\mcA_\Om$, each arc $\alf$ (with endpoints not in $A$) either crosses $A$ or bounces off $A$ in the sense that it misses $\core_{2\mu}(A)$.
%%%%%
%%%%%The ABC property is a fundamental characteristic of hyperbolic and quasihyperbolic geodesics and quasi-geodesics.  \Va\ established this for the quasihyperbolic metric; see \cite[Lemma~3.6]{V-hyp-unif}.  Other metrics with this property include the Ferrand and Kulkarni-Pinkhall-Thurston metrics.  We proved the following in \cite[Proposition~3.8]{HB-geodesics}.
%%%%%
%%%%%%.............................%
%%%%%\begin{fact} \label{F:hk-ABC} %
%%%%%%.............................%
%%%%%In any hyperbolic plane domain:
%%%%%\begin{itemize}
%%%%%  \item[(a)] quasihyperbolic geodesics have the $(\pi,\log2)$-ABC property,
%%%%%  \item[(b)] hyperbolic geodesics have the $(3\KK,5/2)$-ABC property.
%%%%%\end{itemize}
%%%%%\end{fact} %..................%
%%%%%
%%%%%%...........................%
%%%%%\begin{rmks}  \label{R:ABC} %
%%%%%%...........................%
%%%%%It is also true that hyperbolic and quasihyperbolic quasi-geodesics have the ABC property.
%%%%%%%% In fact, quasihyperbolic rough quasi-geodesics have the ABC property.
%%%%%More precisely:
%%%%%
%%%%%\smallskip\noindent(a)  Quasihyperbolic $\Lam$-chordarc paths have the ABC property with the parameters $\mu=\pi\Lam$ and $\nu=\log2$.
%%%%%
%%%%%\smallskip\noindent(b)  Hyperbolic $\Lam$-chordarc paths have the ABC property with the parameters $\mu=7e^\Lam$ and $\nu=5/2$. (Note that $7e>\mu_o:=3\KK$.)
%%%%%%..........%
%%%%%\end{rmks} %
%%%%%%..........%
%%%%%
%%%%%Everywhere below $\mu_o:=\max\{\pi,3\KK,\log16\}=3\KK\le15$.  This absolute constant $\mu_o$ is an ABC parameter for both hyperbolic and quasihyperbolic geodesics.
%%%%%%%%  Henceforth, we reserve the symbol $\mu$ for a general ABC parameter.
%%%%%
%%%%%%-------------------------------------------------------------%
%%%%%\subsection{Distance and Length Estimates}  \label{s:d&l ests}%
%%%%%%-------------------------------------------------------------%
%%%%%We tacitly use the following elementary fact.
%%%%%
%%%%%%:::::::::::::::::::::::::::::::::::%
%%%%%\begin{lma} \label{L:del deep in A} %
%%%%%%:::::::::::::::::::::::::::::::::::%
%%%%%Suppose $A:=\A(o;d,m)\in\mcA_\Om(\log4)$ and $z\in\core_{\log2}(A)$; so $m>\log2$ and $z\in\A(o;d,m-\log2)$.  Then
%%%%%\[
%%%%%  \B(z)\subset\D[o;de^{-m}] \quad\biggl(\text{i.e., for all $\zeta\in\bOm$ with $\del(z)=|z-\zeta|$, $|\zeta-o|\le d e^{-m}$}\biggr)
%%%%%\]
%%%%%and moreover $\ds\half\,|z-o|\le\del(z)\le|z-o|$.
%%%%%\end{lma} %:::::::::::::::::::::::::%
%%%%%%%%%>>>>>>>>>>>>%
%%%%%%%%\begin{proof}%
%%%%%%%%%>>>>>>>>>>>>%
%%%%%%%%Assume $o=0$ and $d=1$.  Then $\del(z)\le|z|<e^{m-\log2}=e^m-e^{m-\log2}$, so any $\zeta\in\B(z)$ must lie outside $\A(o;d,m)$ and hence $|\zeta|\le e^{-m}=de^{-m}$.  Therefore
%%%%%%%%\[
%%%%%%%%  \del(z)=|z-\zeta|\ge|z|-e^{-m}\ge\half\,|z|\,.  \qedhere
%%%%%%%%\]
%%%%%%%%%%%\begin{gather*}
%%%%%%%%%%%  \del(z)\le|z|<e^{m-\log2}=e^m-e^{m-\log2}\,,
%%%%%%%%%%%  \intertext{so any $\zeta\in\B(z)$ must lie outside $\A(o;d,m)$ and hence $|\zeta|\le e^{-m}=de^{-m}$.  Therefore}
%%%%%%%%%%%  \del(z)=|z-\zeta|\ge|z|-e^{-m}\ge\half\,|z|\,.  \qedhere
%%%%%%%%%%%\end{gather*}
%%%%%%%%%<<<<<<<<<<%
%%%%%%%%\end{proof}%
%%%%%%%%%<<<<<<<<<<%
%%%%%
%%%%%Here is a useful consequence of \rf{L:del deep in A}; it says that each of the centers of the two annuli lie inside \emph{both} of the annuli.  We ``see'' fat annuli as punctured disks. \flag{The flwg is ONLY used once at the very end of the Proof of Theorem~A; its cor--not shown--is never used?}
%%%%%
%%%%%%:::::::::::::::::::::::::::::::::::::::::%
%%%%%\begin{lma} \label{L:both centers inside} %
%%%%%%:::::::::::::::::::::::::::::::::::::::::%
%%%%%Assume $r\wedge s>q\ge\log2$.  Let $\A(\eta;d,r),\A(\vth;c,s)\in\mcA_\Om$.  Suppose that $\A(\eta;d,r-q)\cap\A(\vth;c,s-q)\ne\emptyset$.\footnote{These two annuli are the $q$-cores of $\A(\eta;d,r)$ and $\A(\vth;c,s)$, respectively.}  Then
%%%%%%%%\begin{gather*}
%%%%%\[  |\eta-\vth|\le(de^{-r})\wedge(ce^{-s})\,. \]
%%%%%%%%  \intertext{If in addition $\A(\eta;d,r),\A(\vth;c,s)\in\mcA^2_\Om$, then also}
%%%%%%%%  \half\,d \le c \le 2\,d  \quad\text{and}\quad |r-s| \le \log4\,.
%%%%%%%%\end{gather*}
%%%%%If also $\A(\eta;d,r),\A(\vth;c,s)\in\mcA^2_\Om$, then $\ds\half\,d \le c \le 2\,d$ and $|r-s| \le \log4$.
%%%%%\end{lma} %:::::::::::::::::::::::::::::::%
%%%%%%%%%>>>>>>>>>>>>%
%%%%%%%%\begin{proof}%
%%%%%%%%%>>>>>>>>>>>>%
%%%%%%%%Let $z\in\A(\eta;d,r-q)\cap\A(\vth;c,s-q)$ and pick any $\zeta\in\B(z)$.  Then by \rf{L:del deep in A},
%%%%%%%%\[
%%%%%%%%  |\zeta-\eta|\le de^{-r} \quad\text{and}\quad  |\zeta-\vth|\le ce^{-s}\,.
%%%%%%%%\]
%%%%%%%%
%%%%%%%%Suppose $|\eta-\vth|>de^{-r}$.  Then, since $\vth\in\bOm$ and $\A(\eta;d,r)\subset\Om$, $|\eta-\vth|\ge de^{r}$; but now $\vth$ far from $\eta$ means it is also far from $\zeta$ which will cause trouble!  We have
%%%%%%%%\begin{gather*}
%%%%%%%%  ce^{-s} \ge |\zeta-\vth| \ge |\eta-\vth|-|\eta-\zeta| \ge de^r-de^{-r} \ge \half\, d e^r
%%%%%%%%  \intertext{so $de^r\le2ce^{-s}$.  Then, as $|z-\zeta|=\del(z)\le|z-\eta| < de^{r-q}$,}
%%%%%%%%  ce^{-s+q} < |z-\vth| \le |z-\zeta|+|\zeta-\vth| \le d e^{r-q}+ce^{-s} \le (1+2e^{-q})ce^{-s}
%%%%%%%%  \intertext{which implies that $e^q<1+2e^{-q}$.  However, as $q\ge\log2$, this in turn implies the contradiction}
%%%%%%%%  2\le e^q<1+2e^{-q}\le2\,.
%%%%%%%%\end{gather*}
%%%%%%%%
%%%%%%%%Thus $|\eta-\vth|\le de^{-r}$.  Interchanging the roles of $\eta,d,r$ and $\vth,c,s$ we likewise deduce that $|\eta-\vth|\le ce^{-s}$.
%%%%%%%%
%%%%%%%%\medskip
%%%%%%%%
%%%%%%%%Now suppose also that $\A(\eta;d,r),\A(\vth;c,s)\in\mcA^2_\Om$.  Select $\xi_1,\xi_2\in\bOm\cap\bd\A(\eta;d,r)$ with
%%%%%%%%\addtocounter{equation}{1}  % get eqn label below to be correct
%%%%%%%%\begin{gather*}
%%%%%%%%  |\xi_1-\eta|=de^{-r}  \quad\text{and}\quad  |\xi_2-\eta|=de^{r}\,.
%%%%%%%%  \intertext{Below we verify that $\xi_1$ and $\xi_2$ are, respectively, inside and outside $\A(\vth;c,s)$; i.e.,}
%%%%%%%%  |\xi_1-\vth|\le ce^{-s}  \quad\text{and}\quad  |\xi_2-\vth|\ge ce^{s}\,.   \tag{\theequation}\label{E:in n out}
%%%%%%%%\end{gather*}
%%%%%%%%Assuming \eqref{E:in n out} (for now), we proceed as follows.
%%%%%%%%
%%%%%%%%Since $\xi_1,\eta\in\D[\vth;ce^{-s}]$, $de^{-r}=|\xi_1-\eta|\le2ce^{-s}$.  Also,
%%%%%%%%\begin{gather*}
%%%%%%%%  ce^s \le |\xi_2-\vth| \le |\xi_2-\eta|+|\eta-\vth| \le de^r+de^{-r} \le 2de^r\,.
%%%%%%%%  \intertext{Thus}
%%%%%%%%  ce^s \le 2de^r \quad\text{and}\quad de^{-r} \le 2ce^{-s}\,.
%%%%%%%%  \intertext{Interchanging the roles of $\eta,d,r$ and $\vth,c,s$ we likewise deduce}
%%%%%%%%  de^r \le 2ce^s \quad\text{and}\quad ce^{-s} \le 2de^{-r}\,.
%%%%%%%%  \intertext{Therefore,}
%%%%%%%%  d^2=(de^r)(de^{-r})\le(2ce^s)(2ce^{-s})=4c^2\,, \quad\text{so $d\le2c$}.
%%%%%%%%  \intertext{Similarly, $c\le2d$.  Also,}
%%%%%%%%  e^{s-r}\le 2(c/d) \le 4 \quad\text{and}\quad e^{r-s}\le4\,.
%%%%%%%%\end{gather*}
%%%%%%%%
%%%%%%%%\medskip
%%%%%%%%It remains to verify \eqref{E:in n out}.  Since $\xi_i\in\bOm$ while $\A(\vth;c,s)\subset\Om$, either $|\xi_i-\vth|\le ce^{-s}$ or $|\xi_i-\vth|\ge ce^{s}$.
%%%%%%%%Recall that $z\in\A(\eta;d,r-q)\cap\A(\vth;c,s-q)$.
%%%%%%%%
%%%%%%%%Suppose $|\xi_2-\vth|\le ce^{-s}$.  Then $\xi_2,\eta\in\D[\vth;ce^{-s}]$, so $de^r=|\xi_2-\eta|\le2ce^{-s}$.  Thus
%%%%%%%%\begin{gather*}
%%%%%%%%  |z-\eta| < de^{r-q} \le 2ce^{-s-q}
%%%%%%%%  \intertext{whence}
%%%%%%%%  c e^{q-s} < |z-\vth| \le |z-\eta|+|\eta-\vth| < 2ce^{-s-q} + ce^{-s}
%%%%%%%%\end{gather*}
%%%%%%%%which implies the contradiction $e^q<1+2e^{-q}$ (as described above).  Thus, $|\xi_2-\vth|\ge ce^{s}$.
%%%%%%%%
%%%%%%%%Now suppose $|\xi_1-\vth|\ge ce^{s}$.  Then
%%%%%%%%\begin{gather*}
%%%%%%%%  de^{-r} = |\xi_1-\eta| \ge |\xi_1-\vth|-|\vth-\eta| \ge ce^{s} - ce^{-s} \ge \half\,ce^s\,.
%%%%%%%%  \intertext{Therefore}
%%%%%%%%  \half\, c e^{s+q} \le de^{q-r} < |z-\eta| \le |z-\vth|+|\vth-\eta| < ce^{s-q} + ce^{-s}
%%%%%%%%\end{gather*}
%%%%%%%%which again implies the contradiction $e^q<1+2e^{-q}$.  So, $|\xi_1-\vth|\le ce^{-s}$.
%%%%%%%%%<<<<<<<<<<%
%%%%%%%%\end{proof}%
%%%%%%%%%<<<<<<<<<<%
%%%%%
%%%%%%%%%::::::::::::::::::::::::::::::::::::%
%%%%%%%%\begin{cor} \label{C:cores disjoint} %
%%%%%%%%%::::::::::::::::::::::::::::::::::::%
%%%%%%%%Assume $\sig>0$ and $r\wedge s\ge\log3\vee(\sig+\frac13\log3)$.  Let $A:=\A(\eta;d,r)$ and $B:=\A(\vth;c,s)$ be annuli in $\mcA_\Om$.  Suppose there exist points $a,b$ with
%%%%%%%%\begin{center}
%%%%%%%%  $a$ inside \& $b$ outside $\core_\sig(A)$ \hspace{1em}and\hspace{1em} $b$ inside \& $a$ outside $\core_\sig(B)$\,.
%%%%%%%%\end{center}
%%%%%%%%Then $\core_{\log2}(A)\cap\core_{\log2}(B)=\emptyset$\,.
%%%%%%%%\end{cor} %::::::::::::::::::::::::::%
%%%%%%%%%>>>>>>>>>>>>%
%%%%%%%%\begin{proof}%
%%%%%%%%%>>>>>>>>>>>>%
%%%%%%%%Suppose that
%%%%%%%%\begin{gather*}
%%%%%%%%  \core_{\log2}(A)\cap\core_{\log2}(B)\ne\emptyset \quad\text{(i.e., $\A(\eta;d,r-\log2)\cap\A(\vth;c,s-\log2)\ne\emptyset$)}\,.
%%%%%%%%  \intertext{Appealing to \rf{L:both centers inside} we can assert that}
%%%%%%%%  |\eta-\vth|\le(d e^{-r})\wedge(c e^{-s}) \le (c\wedge d) e^{-\tau} \le \frac{c}3\,.
%%%%%%%%  \intertext{Then, as $b$ is outside $\core_\sig(A)$ and inside $\core_\sig(B)$,}
%%%%%%%%  d e^{\tau-\sig} \le d e^{r-\sig} \le |b-\eta| \le |b-\vth|+|\eta-\vth| \le c e^{\sig-s} + |\eta-\vth|\,,
%%%%%%%%  \intertext{so}
%%%%%%%%  d\le c e^{2\sig-\tau-s}+e^{\sig-\tau}|\eta-\vth| \le c e^{2(\sig-\tau)} + e^{\sig-\tau}|\eta-\vth|\,.
%%%%%%%%\end{gather*}
%%%%%%%%Therefore, since $a$ is inside $\core_\sig(A)$,
%%%%%%%%\begin{align*}
%%%%%%%%  |a-\vth| &\le |a-\eta|+|\eta-\vth| \le d e^{\sig-r} + |\eta-\vth|  \\
%%%%%%%%           &\le e^{\sig-\tau} \lp c e^{2(\sig-\tau)} + e^{\sig-\tau}|\eta-\vth| \rp + |\eta-\vth|   \\
%%%%%%%%           &= c e^{3(\sig-\tau)} + e^{2(\sig-\tau)}|\eta-\vth| + |\eta-\vth| < c\,.
%%%%%%%%\end{align*}
%%%%%%%%However, as $a$ lies outside $\core_\sig(B)$, we now have $c>|a-\vth|\ge c e^{s-\sig}$, and this implies the contradiction $\tau>\sig>s\ge\tau$.
%%%%%%%%%<<<<<<<<<<%
%%%%%%%%\end{proof}%
%%%%%%%%%<<<<<<<<<<%
%%%%%
%%%%%
%%%%%%%% flwg all replaced with \rf{C:1in1out}
%%%%%%%%
%%%%%%%%%::::::::::::::::::::::::::::::::%
%%%%%%%%\begin{lma} \label{L:comp dists} %
%%%%%%%%Let $A\in\mcA(\log3)$ with $A\subset\Om$.  Suppose $x,u\in\bdi A$ and $y,v\in\bdo A$.  Then
%%%%%%%%\begin{gather*}
%%%%%%%%  \half |u-v| \le |x-y| \le 2|u-v|\,.
%%%%%%%%  \intertext{If in addition $A\subset\Om$, then also}
%%%%%%%%  \frac16 l(u,v) \le l(x,y) \le 6l(u,v)\,.
%%%%%%%%\end{gather*}
%%%%%%%%\[
%%%%%%%%  \frac16 l(u,v) \le l(x,y) \le 6l(u,v)\,.
%%%%%%%%\]
%%%%%%%%\end{lma} %::::::::::::::::::::::%
%%%%%%%%%>>>>>>>>>>>>%
%%%%%%%%\begin{proof}%
%%%%%%%%%>>>>>>>>>>>>%
%%%%%%%% first part below  replaced with \rf{C:1in1out}
%%%%%%%%Assume that $A=\A(0;d,m)$, so $2m=\md(A)>\log3$.  Since $\cosh(t)\le2\sinh(t)$ for $t\ge\half\log3$,
%%%%%%%%\begin{gather*}
%%%%%%%%  2d\sinh(m)\le|x-y|\le2d\cosh(m)\le4d\sinh(m)\,.
%%%%%%%%  \intertext{Thus}
%%%%%%%%  |x-y|\le4d\sinh(m)\le2|u-v| \quad\text{and similarly}\quad |u-v|\le2|x-y|\,.
%%%%%%%%  \intertext{Assume $A\subset\Om$.  Then $\chi:=\chi_{xy}$ lies in $\Om$ so}
%%%%%%%%  l(x,y)\le\ell(\chi)\le3|x-y|\le6|u-v|\le6l(u,v)
%%%%%%%%\end{gather*}
%%%%%%%%and similarly $l(u,v)\le6l(x,y)$.
%%%%%%%%Evidently, $\chi:=\chi_{xy}$ lies in $\Om$ so by \eqref{E:chi qcx}
%%%%%%%%\[
%%%%%%%%  l(x,y)\le\ell(\chi)\le3|x-y|\le6|u-v|\le6l(u,v)
%%%%%%%%\]
%%%%%%%%and similarly $l(u,v)\le6l(x,y)$.
%%%%%%%%%<<<<<<<<<<%
%%%%%%%%\end{proof}%
%%%%%%%%%<<<<<<<<<<%
%%%%%
%%%%%Here we collect some elementary estimates that are nonetheless quite useful.
%%%%%
%%%%%%:::::::::::::::::::::::::::::%
%%%%%\begin{lma} \label{L:1in1out} %
%%%%%%:::::::::::::::::::::::::::::%
%%%%%Let $A:=\A(o;d,m)$.  Suppose $a,b\in\mfC\sm A$ with $a$ inside $A$ and $b$ outside $A$.  Then $|a-b|\eqx|b-o|$.  More precisely,
%%%%%\[
%%%%%  (1-e^{-2m})|b-o|\le|a-b|\le(1+e^{-2m})|b-o|\,.
%%%%%\]
%%%%%\end{lma} %:::::::::::::::::::%
%%%%%%>>>>>>>>>>>>%
%%%%%\begin{proof}%
%%%%%%>>>>>>>>>>>>%
%%%%%Assume $o=0$.  Then $|a|\le de^{-m}$ and $|b|\ge de^m$, so
%%%%%\begin{gather*}
%%%%%  |a-b|\le|a|+|b|\le de^{-m}+|b|\le(1+e^{-2m})|b|
%%%%%  \intertext{and}
%%%%%  |a-b|\ge|b|-|a|\ge|b|-de^{-m}\ge(1-e^{-2m})|b|\,.
%%%%%\end{gather*}
%%%%%%<<<<<<<<<<%
%%%%%\end{proof}%
%%%%%%<<<<<<<<<<%
%%%%%
%%%%%%:::::::::::::::::::::::::::::%
%%%%%\begin{cor} \label{C:1in1out} %
%%%%%%:::::::::::::::::::::::::::::%
%%%%%Let $A:=\A(o;d,m)\in\mcA(\log3)$.  Suppose $a,a',b,b'\in\mfC\sm A$ with $a,a'$ inside $A$, $|a-o|=|a'-o|$, $b,b'$ outside $A$, $|b-o|=|b'-o|$.  Then $|a-b|\eqx|a'-b'|$.  More precisely,
%%%%%\begin{gather*}
%%%%%  \half|a-b|\le|a'-b'|\le2|a-b|\,.
%%%%%  \intertext{If in addition $B:=\{z\in\mfC\mid |a-o|\le|z-o|\le|b-o|\} \subset\Om$, then also}
%%%%%  \frac16\, l(a,b) \le l(a',b') \le 6\,l(a,b)\,.
%%%%%\end{gather*}
%%%%%\end{cor} %:::::::::::::::::::%
%%%%%%>>>>>>>>>>>>%
%%%%%\begin{proof}%
%%%%%%>>>>>>>>>>>>%
%%%%%%%% first part holds bcuz (1+e^{-2m})(1-e^{-2m})^{-1}\le 2
%%%%%To check the length inequalities, assume $B\subset\Om$.  Then $\chi:=\chi_{ab}$ lies in $\Om$, so by \eqref{E:chi qcx}
%%%%%\[
%%%%%  l(a,b)\le\ell(\chi)\le3|a-b|\le6|a'-b'|\le6l(a',b')
%%%%%\]
%%%%%and similarly $l(a',b')\le6l(a,b)$.
%%%%%%<<<<<<<<<<%
%%%%%\end{proof}%
%%%%%%<<<<<<<<<<%
%%%%%
%%%%%%::::::::::::::::::::::::::::::%
%%%%%\begin{lma} \label{L:comp ell} %
%%%%%%::::::::::::::::::::::::::::::%
%%%%%Let $A:=\A(o;d,m)\in\mcA_\Om(\log4)$.  Suppose $z,z'\in\mfS^1(o;r)\subset\overline\core_{\log2}(A)$; so, $|z-o|=|z'-o|=r\in[2de^{-m},2^{-1}de^m]$.  Then for all $a\in\Om\sm A$, $l(a,z)\eqx\l(a,z')$.  More precisely,
%%%%%\[
%%%%%  \forall\, a\in\Om\sm A\,, \quad (1+2\pi)^{-1} l(a,z)\le\l(a,z')\le (1+2\pi)l(a,z)\,.
%%%%%\]
%%%%%\end{lma} %:::::::::::::::::::%
%%%%%%>>>>>>>>>>>>%
%%%%%\begin{proof}%
%%%%%%>>>>>>>>>>>>%
%%%%%Clearly $l(z,z')\le\pi r$.  Also, for $w\in\{z,z'\}$,
%%%%%\begin{gather*}
%%%%%  l(a,w) \ge \begin{cases}
%%%%%               d e^m - r \quad&\text{if $a$ is outside $A$},\\
%%%%%               r -de^{-m} \quad&\text{if $a$ is inside $A$},
%%%%%             \end{cases}
%%%%%  \quad\text{so}\quad l(a,w)\ge \half\,r\,.
%%%%%  \intertext{Thus $l(z,z')\le\pi r\le2\pi l(a,w)$, and therefore}
%%%%%  l(a,z')\le l(a,z)+l(z,z')\le(1+2\pi)l(a,z) \quad\text{and}\quad l(a,z)\le(1+2\pi)l(a,z')\,.  \qedhere
%%%%%\end{gather*}
%%%%%%<<<<<<<<<<%
%%%%%\end{proof}%
%%%%%%<<<<<<<<<<%
%%%%%

